An unconditionally stable space-time isogeometric method for the acoustic wave equation

We study space--time isogeometric discretizations of the linear acoustic wave equation that use splines of arbitrary degree p, both in space and time. We propose a space--time variational formulation that is obtained by adding a non-consistent penalty term of order 2p+2 to the bilinear form coming from integration by parts. This formulation, when discretized with tensor-product spline spaces with maximal regularity in time, is unconditionally stable: the mesh size in time is not constrained by the mesh size in space. We give extensive numerical evidence for the good stability, approximation, dissipation and dispersion properties of the stabilized isogeometric formulation, comparing against stabilized finite element schemes, for a range of wave propagation problems with constant and variable wave speed.

==> Chapters/Space_time_fem.tex <==
{\color{red}
\subsection{Space-time finite element method}
For a conforming tensor--product space--time piecewise-linear finite element discretization of \eqref{abstractvar}, let us restrict ourselves to consider $\Omega \subset \mathbb{R}^d$ for $d =1,2,3$ and let us assume that $\Omega$ is an interval for $d=1$, or $\Omega$ is a polygon for $d=2$, or $\Omega$ is a polyhedral for $d=3$. Let us define the spatial finite element space as follows
\begin{equation}\label{discrspacefeminspace}
	V_{h_x,0}(\Omega) \subset H^1_0(\Omega),
\end{equation}
which is the space of continuous functions that are piecewise-linear, or piecewise-multilinear, on a uniform admissible decomposition of $\overline{\Omega}$ in intervals $(d=1)$, triangles or quadrilaterals $(d=2)$, and tetrahedra or hexahedra $(d=3)$, with uniform mesh-size $h_x$. Let us define the temporal finite element space as follows
\begin{equation*}
	S^1_{h_t}(0,T) \subset H^1(0,T),
\end{equation*}
which is the space of univariate continuous piecewise-linear functions on a uniform decomposition of $[0,T]$ with mesh-size $h_t$. In this setting, $h$ denotes the space-time mesh-size, i.e., $h := \max{\{h_x,h_t\}}$. Then, let us define the tensor--product space--time finite element space
\begin{equation*}
	Q_h^1(Q) := V_{h_x,0}(\Omega) \otimes S^1_{h_t}(0,T),
\end{equation*}  
As discrete trial and test finite element spaces let us define, respectively, 
\begin{gather}
	\mathcal{W}_h := Q_h^1(Q) \cap H^{1,1}_{0;0,*}(Q) = V_{h_x,0}(\Omega) \otimes \{w_{h_t} \in S^1_{h_t}(0,T) : \ w_{h_t}(0)=0 \}, \label{femtrial}\\
	\mathcal{V}_h := Q_h^1(Q) \cap H^{1,1}_{0;*,0}(Q) = V_{h_x,0}(\Omega) \otimes \{v_{h_t} \in S^1_{h_t}(0,T) : \ v_{h_t}(T)=0 \}. \label{femtest}
\end{gather}
The Petrov-Galerkin finite element discretization of the variational formulation \eqref{abstractvar} reads:
\begin{equation}\label{femwave}
	\text{Find } u_h \in \mathcal{W}_h \text{ such that } a(u_h,v_h)=\mathcal{F}(v_h) \quad \text{for all } v_h \in \mathcal{V}_h.
\end{equation}
The tensor-product structure of the finite element spaces \eqref{femtrial}, \eqref{femtest} allows to write the system matrix $K_h$ as sum of Kronecker products of matrices as
\begin{equation}\label{stifffem}
	K_h := -A_{h_t} \otimes M_{h_x} + M_{h_t} \otimes A_{h_x} \in \mathbb{R}^{N_t \cdot N_x \times N_t \cdot N_x},
\end{equation}
where $M_{h_x},A_{h_x} \in \mathbb{R}^{N_x \times N_x}$ are the spatial mass and stiffness matrix, and $M_{h_t},A_{h_t} \in \mathbb{R}^{N_t \times N_t}$ are the temporal mass and stiffness matrix, respectively.

The space-time Galerkin method \eqref{femwave} is only conditionally stable, as proved in \cite{SZ2020, Z2020}. In fact, stability of the numerical scheme that results from the stiffness matrix \eqref{stifffem} holds only if the CFL condition
\begin{equation}\label{CFL}
	h_t \leq C \hspace{0.05cm} h_x
\end{equation}
is satisfied, where the constant $C > 0$ depends on the constant of a spatial inverse inequality (see \cite[(4.52)]{Z2020}). 
\begin{remark}
	Let the spatial discrete space $V_{h_x,0}(\Omega)$ to be of tensor-product structure with uniform mesh sizes $h_{x_1},\ldots,h_{x_d}$. Let $h_{x,\text{min}}:=\min{\{h_{x_1},\ldots,h_{x_d}\}}$. As stated in \cite{Z2020}, the CFL condition \eqref{CFL} results in
	\begin{equation*}
		h_t \leq \frac{h_{x,\text{min}}}{\sqrt{d}}.
	\end{equation*} 
\end{remark}

To overcome the CFL condition \eqref{CFL}, and by following Zlotnik's idea \cite{Zl1994}, in \cite{SZ2019,Z2020} the authors replace the discrete Galerkin method \eqref{femwave} with the following scheme:

\begin{equation}\label{stabfemwave}
	\text{Find } u_h \in \mathcal{W}_h \text{ such that } a_h(u_h,v_h)=\mathcal{F}(v_h) \quad \text{for all } v_h \in \mathcal{V}_h,
\end{equation}
where the bilinear form $a_h(\cdot,\cdot):  \mathcal{W}_h \times \mathcal{V}_h \rightarrow \mathbb{R}$ is defined as
\begin{equation}\label{stabwaveform}
	a_h(w_h,v_h) := \int_{(0,T)} \int_\Omega \Big[- \partial_t w_h(x,t) \partial_t v_h(x,t) + \nabla_x w_h(x,t) \cdot \big(Q_{h_t}^0\nabla_x v_h\big)(x,t)\Big] \hspace{0.1cm} d\Omega \hspace{0.05cm} dt,
\end{equation}
for $w_h \in \mathcal{W}_h$, $v_h \in \mathcal{V}_h$, and, by denoting with $S^0_{h_t}(0,T)$ the space of piecewise-constant functions on $(0,T)$, the operator
\begin{equation*}
	Q_{h_t}^0: L^2(Q) \longrightarrow L^2(\Omega) \otimes S_{h_t}^0(0,T)
\end{equation*}
defines the extended $L^2$-orthogonal projection onto the space of piecewise-constant functions with respect to time, which acts component-wise in \eqref{stabwaveform}. As a result, unconditional stability and optimal convergence rates are proved in \cite{SZ2019,Z2020}, as summarised in the following Theorem.
\begin{theorem}\cite[Theorem 1.2]{Z2021}\label{theostabfem}
	There exists a unique solution of \eqref{stabfemwave} satisfying the $L^2(Q)$-stability estimate
	\begin{equation*}
		\|u_h\|_{L^2(Q)} \leq \frac{4}{\pi} T^2 \|f\|_{L^2(Q)}.
	\end{equation*}
	Furthermore, if the solution $u$ of \eqref{abstractvar} and $\Omega$ are sufficiently regular, then the unique solution $u_h$ of \eqref{stabfemwave} fulfils the space-time error estimates
	\begin{align*}
		\|u-u_h\|_{L^2(Q)} &\leq Ch^2,\\
		|u-u_h|_{H^1(Q)} &\leq Ch,
	\end{align*}
	where, for the $H^1(Q)$-error estimate, a spatial inverse inequality is additionally assumed.
\end{theorem}	

\begin{remark}
	Theorem \ref{theostabfem} still holds for nonuniform meshes, where $h_x$ and $h_t$ denote the maximum mesh-size in space and time, respectively, and $h := \max{\{h_x,h_t\}}$. For more details see \cite{Z2020}.
\end{remark}

Let us assume to consider nonuniform meshes in space and time. The following Theorem is a key result to define a stable isogeometric method for the wave equation, as it will be clear in Section~\ref{sec:st_iga}.

\begin{prop}\label{prop:stabilization_fem}
	Let $\{\tau_\ell\}_{\ell=1, \ldots,N^{\text{el}}_{t}}$ be the time-elements of the finite element mesh on $(0,T)$. Let $a(\cdot,\cdot)$ be the bilinear form of the abstract variational problem \eqref{abstractvar}.
	The stable discrete bilinear form \eqref{stabwaveform} admits the following equivalent representation
	\begin{equation}\label{equivstab}
		a_h(w_h,v_h) = a(w_h,v_h)- \frac{1}{12} \sum_{\ell=1}^{N^{\text{el}}_{t}} h^2_{t,\ell} \int_{\Omega \times \tau_\ell} \partial_t\nabla_x w_h(x,t) \cdot \partial_t\nabla_x v_h(x,t) \hspace{0.1cm} d\Omega \hspace{0.05cm} dt 
	\end{equation}
	for $w_h \in \mathcal{W}_h$, $v_h \in \mathcal{V}_h$. 
\end{prop}

\begin{proof}
	Equality \eqref{equivstab} is a straightforward consequence of \cite[Lemma 17.7]{SZ2019}.
\end{proof}}
